Cartesian Factorization Systems and Grothendieck Fibrations

Every Grothendieck fibration gives rise to a vertical/cartesian orthogonal factorization system on its domain. We define a cartesian factorization system to be an orthogonal factorization in which the left class satisfies 2-of-3 and is closed under pullback along the right class. We endeavor to show that this definition abstracts crucial features of the vertical/cartesian factorization system associated to a Grothendieck fibration, and give comparisons between various 2-categories of factorization systems and Grothendieck fibrations to demonstrate this relationship. We then give a construction which corresponds to the fiberwise opposite of a Grothendieck fibration on the level of cartesian factorization systems. Apart from the final double categorical results, this paper is entirely review of previously established material. It should be read as an expository note.

==> preamble.tex <==
\usepackage{fullpage}
\usepackage{fancyhdr}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{wrapfig} %
\usepackage{graphicx} %
\usepackage{tikz-cd}
\usepackage[margin=1.3in]{geometry} %
\usepackage[backend=biber]{biblatex}
\usepackage{tipa} %
\usepackage{mathtools} %
\usepackage{caption}
\usepackage{hyperref}
\usepackage[capitalize]{cleveref}
\usepackage{thmtools, thm-restate} %

\RequirePackage{hyperref}
\hypersetup{colorlinks,linkcolor={blue!50!black},citecolor={red!50!black},urlcolor={blue!80!black}}

\usetikzlibrary{decorations.pathreplacing} %

\newlength{\perspective} %

\graphicspath{graphics/}

%
\newcounter{nodemaker}
\setcounter{nodemaker}{0}
\def\twocell#1{%
  \global\edef\mynodeone{twocell\arabic{nodemaker}}%
  \stepcounter{nodemaker}%
  \global\edef\mynodetwo{twocell\arabic{nodemaker}}%
  \stepcounter{nodemaker}%
  \ar[#1,phantom,shift left=3,""{name=\mynodeone}]%
  \ar[#1,phantom,shift right=3,""'{name=\mynodetwo}]%
  \ar[Rightarrow,from=\mynodeone,to=\mynodetwo]%
}
%
\DeclareMathOperator{\Aa}{\mathcal{A}}
\DeclareMathOperator{\Ba}{\mathcal{B}}
\DeclareMathOperator{\Ca}{\mathcal{C}}
\DeclareMathOperator{\Da}{\mathcal{D}}
\DeclareMathOperator{\Ea}{\mathcal{E}}
\DeclareMathOperator{\Fa}{\mathcal{F}}
\DeclareMathOperator{\Ga}{\mathcal{G}}
\DeclareMathOperator{\Ha}{\mathcal{H}}
\DeclareMathOperator{\Ka}{\mathcal{K}}
\DeclareMathOperator{\La}{\mathcal{L}}
\DeclareMathOperator{\Ma}{\mathcal{M}}
\DeclareMathOperator{\Na}{\mathcal{N}}
\DeclareMathOperator{\Oa}{\mathcal{O}}
\DeclareMathOperator{\Pa}{\mathcal{P}}
\DeclareMathOperator{\Qa}{\mathcal{Q}}
\DeclareMathOperator{\Ra}{\mathcal{R}}
\DeclareMathOperator{\Sa}{\mathcal{S}}
\DeclareMathOperator{\Ta}{\mathcal{T}}
\DeclareMathOperator{\Ua}{\mathcal{U}}
\DeclareMathOperator{\Va}{\mathcal{V}}
\DeclareMathOperator{\Wa}{\mathcal{W}}
\DeclareMathOperator{\Xa}{\mathcal{X}}
\DeclareMathOperator{\Ya}{\mathcal{Y}}
\DeclareMathOperator{\Za}{\mathcal{Z}}

%
\DeclareMathOperator{\Ab}{\mathbb{A}}
\DeclareMathOperator{\Bb}{\mathbb{B}}
\DeclareMathOperator{\Cb}{\mathbb{C}}
\DeclareMathOperator{\Db}{\mathbb{D}}
\DeclareMathOperator{\Eb}{\mathbb{E}}
\DeclareMathOperator{\Fb}{\mathbb{F}}
\DeclareMathOperator{\Gb}{\mathbb{G}}
\DeclareMathOperator{\Hb}{\mathbb{H}}
\DeclareMathOperator{\Kb}{\mathbb{K}}
\DeclareMathOperator{\Lb}{\mathbb{L}}
\DeclareMathOperator{\Mb}{\mathbb{M}}
\DeclareMathOperator{\Nb}{\mathbb{N}}
\DeclareMathOperator{\Ob}{\mathbb{O}}
\DeclareMathOperator{\Pb}{\mathbb{P}}
\DeclareMathOperator{\Qb}{\mathbb{Q}}
\DeclareMathOperator{\Rb}{\mathbb{R}}
\DeclareMathOperator{\Sb}{\mathbb{S}}
\DeclareMathOperator{\Tb}{\mathbb{T}}
\DeclareMathOperator{\Ub}{\mathbb{U}}
\DeclareMathOperator{\Vb}{\mathbb{V}}
\DeclareMathOperator{\Wb}{\mathbb{W}}
\DeclareMathOperator{\Xb}{\mathbb{X}}
\DeclareMathOperator{\Yb}{\mathbb{Y}}
\DeclareMathOperator{\Zb}{\mathbb{Z}}

\DeclareMathOperator{\pc}{\mathfrak{p}}
\DeclareMathOperator{\Ic}{\mathfrak{I}}
\DeclareMathOperator{\bang}{^^21}

%
\DeclareMathOperator{\im}{\mathsf{im}}
\DeclareMathOperator{\Hom}{\mathsf{Hom}}
\DeclareMathOperator{\Spec}{\mathsf{Spec}}
\DeclareMathOperator{\Gr}{\mathsf{Gr}}
\DeclareMathOperator{\join}{\vee}
\DeclareMathOperator{\meet}{\wedge}

%
\DeclareMathOperator{\op}{^\textnormal{op}}
\DeclareMathOperator{\inv}{^{-1}}
\DeclareMathOperator{\id}{\mathsf{id}}
\renewcommand{\ker}{\mathsf{ker}}
\DeclareMathOperator{\coker}{\mathsf{coker}}
\DeclareMathOperator{\Aut}{\mathsf{Aut}}
\DeclareMathOperator{\BAut}{\mathsf{BAut}}
\DeclareMathOperator{\Map}{\mathsf{Map}}
\DeclareMathOperator{\Gal}{\mathsf{Gal}}
\DeclareMathOperator{\colim}{\mathsf{colim}}
\DeclareMathOperator{\End}{\mathsf{End}}
\DeclareMathOperator{\Dir}{\type{Dir}}
\DeclareMathOperator{\Poly}{\type{Poly}}
\DeclareMathOperator{\Fun}{\type{Fun}}
\DeclareMathOperator{\ext}{\term{ext}}
\DeclareMathOperator{\DirSeries}{\type{DirSeries}}
\DeclareMathOperator{\dom}{\term{dom}}
\DeclareMathOperator{\cod}{\term{cod}}

%
\DeclareMathOperator{\ev}{\textbf{ev}}
\DeclareMathOperator{\Prop}{\textbf{Prop}}
\DeclareMathOperator{\Type}{\textbf{Type}}
\DeclareMathOperator{\precomp}{^{\ast}}
\DeclareMathOperator{\postcomp}{_{\ast}}
\DeclareMathOperator{\refl}{\mathsf{refl}}
\DeclareMathOperator{\fib}{\mathsf{fib}}
\DeclareMathOperator{\cofib}{\type{cofib}}
\DeclareMathOperator{\Zero}{\textbf{0}}
\DeclareMathOperator{\One}{\textbf{1}}
\DeclareMathOperator{\fst}{\term{fst}}
\DeclareMathOperator{\snd}{\term{snd}}
\DeclareMathOperator{\base}{\term{base}}
\DeclareMathOperator{\funext}{\term{funext}}
\DeclareMathOperator{\tr}{\term{tr}}
\DeclareMathOperator{\ap}{\term{ap}}
\DeclareMathOperator{\at}{\term{\, at\,}}
\DeclareMathOperator{\glue}{\term{glue}}
\DeclareMathOperator{\inl}{\term{inl}}
\DeclareMathOperator{\inr}{\term{inr}}
\DeclareMathOperator{\esh}{\text{\textesh}}
\let\bang\relax %
\DeclareMathOperator{\bang}{!}
\DeclareMathOperator{\defin}{\term{-def}}
\DeclareMathOperator{\Bool}{\textbf{Bool}}
\newcommand{\sslash}{\mathbin{/\mkern-6mu/}} %

%
\DeclareMathOperator{\Set}{\type{Set}}
\DeclareMathOperator{\Top}{\textbf{Top}}
\DeclareMathOperator{\Grph}{\textbf{Grph}}
\DeclareMathOperator{\AbCat}{\textbf{Ab}}
\DeclareMathOperator{\Cat}{\textbf{Cat}}
\DeclareMathOperator{\Vect}{\textbf{Vect}}
\DeclareMathOperator{\Ring}{\textbf{Ring}}
\DeclareMathOperator{\Mod}{\textbf{Mod}}
\DeclareMathOperator{\Alg}{\textbf{Alg}}
\DeclareMathOperator{\Aff}{\textbf{Aff}}
\DeclareMathOperator{\SqFree}{\textbf{SqFree}}
\DeclareMathOperator{\SQC}{\Alg_{\textbf{SQC}}}


%
\newcommand{\wlim}[1]{\lim\nolimits_{#1}\!}
\newcommand{\wcolim}[1]{\text{colim}_{#1}}
\newcommand{\yo}{\type{y}}

%
%
%

%
\newcommand{\lam}[1]{\lambda {#1}.\,}       %
\newcommand{\dprod}[1]{({#1}) \to }           %
\newcommand{\dsum}[1]{({#1}) \times }       %
\newcommand{\type}[1]{\mathsf{{#1}}}
\newcommand{\term}[1]{\mathsf{{#1}}}
\newcommand{\ax}[1]{\mathsf{{#1}}}
\newcommand{\trunc}[1]{\left\lVert#1\right\rVert}       %
\newcommand{\ph}{\vphantom{)}} %
\newcommand{\BB}{\term{B}}
\newcommand{\pt}{\term{pt}}
\newcommand{\const}{\term{const}}

%
\newcommand{\xto}[1]{\xrightarrow{#1}}
\newcommand{\todot}{\xrightarrow{\bullet}}
\newcommand{\pto}{\,\cdot\kern-.1em{\to}\,}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\mono}{\rightarrowtail}

%
\newcommand{\prism}{\mathsf{Prism}}
\newcommand{\ob}{\mathsf{ob}}
\newcommand{\Finset}{\mathsf{Finset}}
\newcommand{\TFS}{\mathsf{TFS}}
\newcommand{\Lens}{\mathsf{Lens}}
\newcommand{\LLens}{\mathsf{LawLens}}
\newcommand{\SLens}{\mathsf{SimpLens}}
\newcommand{\Dyn}{\mathsf{Dyn}}
\newcommand{\lens}[2]{\begin{pmatrix}{#1} \\ {#2} \end{pmatrix}}

%
\newcommand{\an}[1]{{\color{red} #1}}

%
\newcommand{\dis}[1]{{\color{blue} DIS says:\ #1}}
\newcommand{\jaz}[1]{{\color{red} Jaz says:\ #1}}
\newcommand{\down}{\mathbin{\downarrow}}

%
\makeatletter
\providecommand*{\xmapstofill@}{%
  \arrowfill@{\mapstochar\relbar}\relbar\rightarrow
}
\providecommand*{\xmapsto}[2][]{%
  \ext@arrow 0395\xmapstofill@{#1}{#2}%
}

%
\newcommand{\xequals}[1]{\overset{{#1}}{=\joinrel=}}
\newcommand{\equalsdot}{\xequals{\bullet}}

%
\makeatletter
\def\slashedarrowfill@#1#2#3#4#5{%
  $\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
   \relax#5#1\mkern-7mu%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mathclap{#3}\mathclap{#2}%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mkern-7mu#4$%
}
\def\rightslashedarrowfill@{%
  \slashedarrowfill@\relbar\relbar\mapstochar\rightarrow}
\newcommand\xslashedrightarrow[2][]{%
  \ext@arrow 0055{\rightslashedarrowfill@}{#1}{#2}}
\makeatother

\newcommand{\xtopro}[1]{\xslashedrightarrow{#1}} %
\newcommand{\topro}{\xslashedrightarrow{}}

\tikzset{
    vert/.style={anchor=south, rotate=90, inner sep=.5mm}
} %

%
\newcommand{\internal}[1]{\ulcorner{#1}\urcorner}


\newtheorem{thm}{Theorem}[section]

%
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{tentative}[thm]{Tentative Definition}
\newtheorem{principle}{Principle}
\newtheorem{question}{Question}
\newtheorem{ex}{Example}
\newtheorem{axiom}{Axiom}
\newtheorem{exercise}{Exercise}[section]
\newtheorem{rmk}[thm]{Remark}
\newtheorem*{solution}{Solution}
\newtheorem*{acknowledgements}{Acknowledgements}


\newtheorem{lem}[thm]{Lemma}
\newtheorem{notation}{Notation}
\newtheorem*{claim}{Claim}
\newtheorem*{fclaim}{False Claim}
\newtheorem{obs}[thm]{Observation}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{con}[thm]{Construction}
